Epidemic Models for COVID-19 during the First Wave from February to May 2020: a Methodological Review

We review epidemiological models for the propagation of the COVID-19 pandemic during the early months of the outbreak: from February to May 2020. The aim is to propose a methodological review that highlights the following characteristics: (i) the epidemic propagation models, (ii) the modeling of intervention strategies, (iii) the models and estimation procedures of the epidemic parameters and (iv) the characteristics of the data used. We finally selected 80 articles from open access databases based on criteria such as the theoretical background, the reproducibility, the incorporation of interventions strategies, etc. It mainly resulted to phenomenological, compartmental and individual-level models. A digital companion including an online sheet, a Kibana interface and a markdown document is proposed. Finally, this work provides an opportunity to witness how the scientific community reacted to this unique situation.

==> glossary/glossary_abbreviations.tex <==
\small

\begin{longtable}{ | p{4cm} | p{2cm} | }

\hline

Term & Shortcut \\
\hline

with respect to & wrt \\
\hline
simulated & $ \sim $ \\
\hline 

\end{longtable}



==> glossary/glossary_epidemio_vocabulary.tex <==
\small

\begin{longtable}{ | p{4cm} | p{7cm} | p{2cm} | }

\hline

Term & Definition & Shortcut \\
\hline

Susceptible state & healthy population without COVID-19 that can be infected if contact with an infectious person & S \\
\hline
Exposed state & exposed to the virus but not infectious & E \\
\hline
Infectious state & symptomatic or asymptomatic population that are supposed infectious (if different definition to precise in the biblio table)
 & I \\
\hline
Recovered / removed state & recovered / removed population from the disease & R \\
\hline
Deceased state & dead population from the disease & D \\
\hline
Quarantine state & placed into quarantine & Q \\
\hline
Hospitalized state & admission in hospital & H \\
\hline
ICU state & admission to ICU & ICU \\
\hline
Basic reproduction number & the average number of secondary infections produced by a typical case of an infection in a population where everyone is susceptible & R0 \\
\hline
Effective reproduction number & It is the average number of secondary infections produced by a typical case of an infection in the current state of a population & Re \\
\hline
Transmission rate & the rate at which infected individuals infect the susceptible population &  \\
\hline
Recovery rate  & the rate at which infected individuals recover &  \\
\hline
Mortality rate & death rate due to the disease &  \\
\hline
Incidence rate & force of infection in the population &  \\
\hline
Latent period & period between exposure and infection &  \\
\hline
Incubation period & period between exposure and onset of clinical symptoms &  \\
\hline
Generation time & when one person transmits an infection to another, time that elapses between onset of symptoms in the primary case and onset of symptoms of the secondary case &  \\
\hline 

\end{longtable}



==> glossary/glossary_institutions,_organizations.tex <==
\small

\begin{longtable}{ | p{4cm} | p{2cm} | }

\hline

Term & Shortcut \\
\hline

World Health Organization & WHO \\
\hline
Center for Disease Control & CDC  \\
\hline
National Health Commission & NHC \\
\hline
Intense Care Unit & ICU \\
\hline
Johns Hopkins University & JHU \\
\hline
Washington State Department of Health & WADoH \\
\hline
Washington Disease Reporting System & WDRS \\
\hline
Système d’Information pour le suivi des VICtimes d’attentats et de situations sanitaires exceptionnelles & SI-VIC \\
\hline 

\end{longtable}



==> glossary/glossary_mathematical_vocabulary.tex <==
\small

\begin{longtable}{ | p{4cm} | p{2cm} | }

\hline

Term & Shortcut \\
\hline

Sum of squared errors & SSE \\
\hline
Mean squared errors & MSE \\
\hline
Root mean squared error & RMSE \\
\hline
Integral square error & ISE \\
\hline
Least Squared estimator & LSE \\
\hline
Maximum likelihood estimation & MLE \\
\hline
Mean Absolute Error & MAE \\
\hline
Fast Fourier Transform & FFT \\
\hline
Ordinary Least Squares & OLS \\
\hline
Finite Impulse Response & FIR \\
\hline
Ordinary Differential Equation & ODE \\
\hline
Inhomogeneous Random Social Network & IRSN \\
\hline
Neural Network & NN \\
\hline
A Framework for Reconstructing Epidemiological Dynamics & FRED \\
\hline
Group of Optimized and Multisource Selection & GROOMS \\
\hline
Gradient Descent & GD \\
\hline
Stochastic Gradient Descent & SGD \\
\hline
Akaike information criterion & AIC \\
\hline
Gauss Error Function & ERF \\
\hline
Bayesian Information Criteria & BIC \\
\hline
Generalized Additive Model & GAM \\
\hline
Generalized Logistic Regression & GLR \\
\hline
Metropolis-Hastings MCMC & MH-MCMC \\
\hline
Hamiltonian Monte-Carlo & HMC \\
\hline
Maximum a Posteriori & MAP \\
\hline
Markov Chain Monte Carlo & MCMC \\
\hline
Approximate Bayesian Computation & ABC \\
\hline 

\end{longtable}



==> glossary/glossary_model_typology.tex <==
\small

\begin{longtable}{ | p{4cm} | p{7cm} |}

\hline

Term & Definition \\
\hline

age-structured & model stratified by age \\
\hline
spatially-structured & model stratified by region, state or country, or other geographical unit \\
\hline 

\end{longtable}



==> review/brouillon_conclusion.tex <==

\bigskip
Analyze the way the scientific community has reacted in the first months:

\begin{itemize}

    \item \textbf{Réactivité scientifique} - Grande réactivité scientifique de la communauté (rapidité + quantité d'études + intégration des problématiques abordées dans la société et le politique). Equipes qui écrivent plusieurs articles successifs, pour améliorer leurs travaux précédents, en prenant en compte les défauts de leurs articles précédents. 
    
    Souligner le fait que beaucoup d'articles ont proposé de nouvelles choses pour s'adapter aux spécificités du covid, par ex modélisation de l'utilité des masques et du confinement qui faisaient polémique, test de différentes stratégies en phase avec les propositions politiques, modélisation des "superpropagateurs", des asymptomatiques, etc...
    
    D'ailleurs articles tellement "dans le coup" qu'ils ont influencé le politique (exemple de l'Imperial college) et étaient suivis de très près (chaque nouvelle étude était citée dans le journal ! Par ex Pasteur etc)
       
    \item \textbf{"Contre-coup" de la réactivité - de l'urgence} : étape de review et publication raccourcie (count the proportion of preprint articles) + relever le fait que peu d'articles font un état de l'art préalable (en général démarrent direct en proposant leur modèle),  peu de comparaison avec les autres épidémies/modèles peu de remise en contexte. Articles manquant de rigueur voire faux (exemple du Lancet) (mais voir si on parle de ça car pas en lien avec les modèles). Certains articles en ont toutefois conscience et prennent des pincettes : article qui a mis un disclaimer pour alerter sur le temps d'écriture très rapide et le manque de recul.
    
    Idée de compter les équipes qui n'étaient pas spécialistes de l'épidémio
 
    \item \textbf{Problème d'accès aux données} - peut-etre dire que lorsqu'on a fait ce projet, les articles qui etaient publiés se basaient sur des données externes soumises à des politiques d'enregistrement différentes. 

    
    \item \textbf{Reproductibilité scientifique} code + reproductibilité - beaucoup de simulations sur internet, efforts pour communiquer à la population, question du travail "collectif" ou des équipes qui font leur truc perso, concerne aussi les données
\end{itemize}

==> review/param_detailed.tex <==


\begin{itemize}
    \item det:\cite{zeng2020predictions} (for the time-dependent functions: virus-contact population per province: closed-formed equations of fixed parameters from public data),  \cite{zheng2020total} (estimation of the vector of compartments rates with dubbed iterative Nelder-Mead to compute the regularized posterior mode), \cite{nadim2020short} (estimation of the threshold rates of exposed and the isolated that are infected through the computation of the partial derivatives of R0 if lockdown, in order to measure the ranges for the interventions scenarios;)
    
    \item MLE: \cite{zheng2020total} (estimation of the vector of compartments rates for 1) MAP of MLE),
    
    
    \item descriptive: \cite{salje2020estimating} (for the relative risk of getting infected for a specific age group: the mean number of contacts that an individual of this age group has on a daily basis as measured in France, weighted by the proportion of the population that is within this age group;), \cite{salje2020estimating} (mean cumulative probability of having been infected across the entire population;)
    
    \item bayesian statistical model\\ 
    Hierarchical model: \cite{flaxman2020report} (generation time distribution; symptoms to death rate distribution; infection to symptoms rate distribution), \cite{li2020substantial} (delay between infection and confirmation of that individual infection for documented infected) via Bayesian inference (Ensemble Adjustment Kalman Filter)) \\
    
    \item regression (especially for the compartments rates): \cite{Thakkar20}, \cite{de2020coronavirus}, \cite{calafiore2020modified}, \cite{yang2020rational}, \cite{nadim2020short}, \cite{Jiwei20}
    
    
    
    
    
    \item likelihood-based methods\\
    \cite{verity2020estimates}(death ratio),  \cite{linton2020incubation} (doubly interval-censored likelihood function with: 1) uniform law of the exposure time variable; 2) pdf of the incubation period chosen as lognormal, Weibull, gamma distributions), \cite{anzai2020assessing} (time delay of a major epidemic:(reduced) hazard of exponential function ),  \cite{roques2020modele} (transmission rate, introduction date, relative rates),\cite{li2020substantial} (transmission rate due to documented infected individuals; multiplicative factor reducing the transmission rate of unreported infected patients; multiplicative factor to adjust mobility data estimates of human movement between cities; fraction of infections that develop severe symptoms (and thus are documented); average latency period; average duration of infection), \cite{zheng2020total} (rates), \cite{roux2020covid} (introduction date and other parameters),  \cite{salje2020estimating} (age-dependent probabilities hospitalization and admission to ICU)\\
    
    Sto micro.. \cite{ZHANGlit2020} (fit a gamma distribution on the generation time + AIC to determine the best fitting), \\
    
    \item AIC-based model selection
    Sto stat \cite{linton2020incubation} (pdf of the incubation period chosen as lognormal, Weibull, gamma distributions; bayesian method with the widely applicable information criterion (WAIC) for model selection; comparison with point estimation outputs from MLE)
    
\end{itemize}





\paragraph{Deterministic methods.}\\

Det comp: \cite{djidjou2020optimal} (disease-induced mortality and transmission rate computed by closed forms deterministic equations),  \cite{chen2020time} ( R0 and isolation rate using Levenberg-Marquad method or MCMC with LSE), \cite{victor2020mathematical} and \cite{Jiwei20} (R0 next-generation matrix method)\\

Sto comp: \cite{zeng2020predictions} (for the time-dependent functions: virus-contact population per province, amount of moving-out population, exposed patients and restriction force: closed-formed equations of fixed parameters from public data),  \cite{zheng2020total} (estimation of the vector of compartments rates for 1) MAP of MLE; 2) and 3) if total variation regularization, dubbed iterative Nelder-Mead to compute the regularized posterior mode), \cite{di2020expected} (R0 next-generation matrix method)\\

Sto stat: \cite{yang2020rational} and \cite{li2020estimation} (R0: exponential growth, which assumes an exponential growth curve to the virus and estimates the R0 from the Lotka-Euler equation;  for the overall estimate of R0: weighted average (weights from a Poisson loss function) of the five previous R0)

\cite{nadim2020short} (estimation of the threshold rates of exposed and the isolated that are infected through the computation of the partial derivatives of R0 if lockdown, in order to measure the ranges for the interventions scenarios;)


\paragraph{Estimators obtained through descriptive methods:}\\
Det comp \cite{salje2020estimating} (for the relative risk of getting infected for a specific age group: the mean number of contacts that an individual of this age group has on a daily basis as measured in France, weighted by the proportion of the population that is within this age group;
)



\paragraph{Estimators obtained through inferential methods.}


\textbf{Bayesian inference.} %Three articles introduce Bayesian statistical model categorised as stochastic, namely a hierarchical model (for key time-to-event intervals distributions in compartmental models) (\cite{flaxman2020report} and \cite{li2020substantial}) and a sequential model to estimated $R_0$ in \cite{li2020estimation}. It leads to regression analysis used through mixed-effects negative-binomial generalized linear model fitted by MCMC in \cite{woody2020projections}.
%Three articles introduce Bayesian statistical model categorised as stochastic, namely a hierarchical model (\cite{flaxman2020report} and \cite{li2020substantial}) and a sequential model, in \cite{li2020estimation}. \\%It leads to regression analysis used through mixed-effects negative-binomial generalized linear model and fitted by MCMC in \cite{woody2020projections}.

%\textbf{Regression Analysis} The majority of articles estimated the parameters by classic frequentist regression analysis. Readers can refer to \cite{woody2020projections} for the only Bayesian regression method, introducing estimation via mixed-effects negative-binomial generalized linear model. Indeed, $2$ articles used OLS (\cite{chen2020scenario}, \cite{chen2020time}) and 

\begin{itemize}

    \item bayesian statistical model\\ 
    Hierarchical model\\
    Sto comp \cite{flaxman2020report} (generation time distribution; symptoms to death rate distribution; infection to symptoms rate distribution: bayesian hierarchical model, parameters are estimated via adaptive HMC), \cite{li2020substantial} (delay between infection and confirmation of that individual infection for documented infected) via Bayesian inference (Ensemble Adjustment Kalman Filter)) \\
        
    Sequential bayes: \cite{li2020estimation}(sequential bayesian method, in which the posterior probability distribution of the R0 is estimated sequentially using the posterior at the previous time point as the new prior;)\\
    
    \item frequentist and bayesian regression analysis\\
    
    
    \textbf{bayesian regression analysis}
    
    Sto pheno: \cite{woody2020projections} (mixed-effects negative-binomial generalized linear model fitted by MCMC)\\ 
    
    \textbf{frequentist regression analysis}
    
   det comp \cite{Thakkar20}(infection rate estimated by regression of movement covariate against case-based estimates)\\
    RMSE:\\
    Det comp: \cite{magdon2020machine} (GD using a combination of RMSE and root-mean-squared-percentage-error between observed dynamics and model predictions), \cite{de2020coronavirus} (compartment rates: optimization via Differential Evolution an optimization technique that randomly creates an initial set of possible solutions and chooses the best one by minimization of RMSE)\\
    MSE:\\
    Sto comp: \cite{chen2020scenario} (regression for R0), \cite{dandekar2020quantifying} (rates of the compartments for SIR, SEIR, estimated by minimization of the MSE loss function through local adjoint sensitivity analysis of the infected and recovered, using the ADAM optimizer. )\\
    Det comp: \cite{calafiore2020modified} (classic parameters (transmission, recovery and mortality rates) estimated via the minimization of a weighted MSE between observed and predicted I, R, D sequences), \cite{chen2020time} ( R0 and isolation rate using Levenberg-Marquad method or MCMC with LSE) \\
    
    LSE: \\
    Sto stat: \cite{covid2020forecasting}(GLM with mixed effects; estimated via nonlinear LSE regression of the cumulative number of deaths, use of L-BFGS-B algorithm), \\
    
    Sto pheno: \cite{yang2020rational} (standard non-linear LSE), \\
    
    Det comp: \cite{nadim2020short} (rates estimated on data with non-linear LSE minimization on Matlab), \cite{Jiwei20} (LSE for suceptible to exposed rate and recovery rate), \cite{Batista20_2} (nonlinear LSE between the actual and predicted number of cases)\\

    
    
    
    OLS/loglinear:\\
    
     Det comp: \cite{chen2020scenario} (country-level fixed in the transmission rate; country-independent effect of intervention parameters on the infection rate; recovery rate for each country), \cite{chen2020time} (R0 and isolation rate using Levenberg-Marquad method or MCMC with LSE)\\
    
    linear regression: Det stat \cite{adiga2020evaluating} (estimation of the beginning date of the epidemic spread per country, univariate linear regression models and Wald test with a t-distribution against a null hypothesis of a slope of 0), Det comp \cite{Thakkar20} (infection rate estimated by regression of movement covariate against case-based estimates)\\
    
   log-linear regression: \cite{li2020estimation} (R0), Sto pheno \cite{verity2020estimates} (prior of growth rate estimated by a log-linear model)\\
   
   
    
    
    
    
    \item likelihood-based methods\\
    Sto pheno \cite{roy2020} (prior distribution of the coefficients of the parameters B-spline decomposition from the likelihood function using HMC algorithm), \cite{verity2020estimates}(prior of growth rate estimated by a log-linear model; death ratio with parametric MAP and nonparametric Kaplan-Meier method)\\
    
    Sto stat \cite{linton2020incubation} (doubly interval-censored likelihood function with: 1) uniform law of the exposure time variable; 2) pdf of the incubation period chosen as lognormal, Weibull, gamma distributions; bayesian method with the widely applicable information criterion (WAIC) for model selection; comparison with point estimation outputs from MLE), \cite{li2020estimation} (Poisson distribution on the number of cases generated from a single case), \cite{anzai2020assessing} (time delay of a major epidemic: hazard of exponential function of a major epidemic in the absence of travel volume changes, reduced hazard of exponential function by the relative reduced probability of a major epidemic, confidence intervals estimated by profile MLE method (SAS) ), \cite{yang2020rational} and \cite{li2020estimation} (R0: MLE method based on the assumption that the number of cases generated from a single case is Poisson distributed and depends on the R0)\\
    
    Sto comp \cite{roques2020modele} (transmission rate, initial date of the epidemic, relative probability to be tested for a susceptible vs an infected; MLE of the increments of the daily new cases $\wrt$ the three parameters to optimize, optimization under constraints, Matlab fmincon function),\cite{li2020substantial} (MLE for the parameters: transmission rate due to documented infected individuals; multiplicative factor reducing the transmission rate of unreported infected patients; multiplicative factor to adjust mobility data estimates of human movement between cities; fraction of infections that develop severe symptoms (and thus are documented); average latency period; average duration of infection), \cite{zheng2020total} (estimation of the vector of compartments rates for 1) MAP of MLE; 2) and 3) if total variation regularization, dubbed iterative Nelder-Mead to compute the regularized posterior mode), \cite{gleam2020modeling} ( sensitivity analysis to select them with Approximate Bayesian Computation and MAP), \cite{chinazzi2020effect} (sensitivity analysis to select them with ABC and MAP)\\
    
    Det comp: \cite{roux2020covid} (introduction date of the virus and other parameters are estimated as MLE assuming some specific distributions for the hospitalization data, the occupation of hospitalization beds, the ICU and deaths data), \cite{leung2020first} (estimate the Re over time (maximum likelihood estimation using the distribution of the generation time) used after MCMC to that estimates the distribution of the time from symptomatic to confirmed dynamic), \cite{leung2020first} (MLE using the distribution of the generation time), \cite{salje2020estimating} (mean cumulative probability of having been infected across the entire population; age-dependent probabilities hospitalization and admission to ICU are fitted by MLE (Poisson distribution on the number of ICU by age and gender, and the number of hospitalizations by age and gender))\\
    
    Sto micro.. \cite{ZHANGlit2020} (MLE to fit a gamma distribution on the generation time, AIC to determine the best fitting), \\
    
    \item AIC-based model selection
    Sto stat \cite{linton2020incubation} (pdf of the incubation period chosen as lognormal, Weibull, gamma distributions; bayesian method with the widely applicable information criterion (WAIC) for model selection; comparison with point estimation outputs from MLE), \cite{chinazzi2020effect} (sensitivity analysis to select them with ABC and MAP), \cite{ZHANGlit2020} (fit a gamma distribution on the generation time + AIC to determine the best fitting)
        
\end{itemize}


\paragraph{Sampling methods.}

\begin{itemize}
    \item bayesian\\
    MCMC:\\
    Sto comp \cite{woody2020projections}, \cite{chen2020time}(R0 and isolation rate using Levenberg-Marquad method or MCMC with LSE), \cite{wu2020nowcasting} (Gibbs sampling and non-informative flat prior)\\
    Sto pheno \cite{roy2020} (prior distribution of the coefficients of the parameters B-spline decomposition from the likelihood function, using HMC algorithm), \cite{verity2020estimates} (onset-to-recovery time $\sim$ gamma distribution; parameters of the Gamma distribution estimated by MCMC), \cite{kraemer2020effect} (incubation period $\sim$ Gamma distribution; mean and variance of the distribution estimated using MCMC), \cite{shim2020transmission}, \\
    
    Det comp \cite{leung2020first}  (distribution on the time of symptoms-to-report), \\ 
    
    
    MH-MCMC:\\
    Sto stat \cite{ZHANGlit2020}(MH-MCMC sampling to estimate the posterior distribution of Re over time), \cite{li2020estimation} (estimation of the R0 from a SEIR model; with the use of a MH-MCMC algorithm)\\
    Det comp \cite{salje2020estimating}  initial number of exposed and mean time spent in ICU are jointly estimated via MH-MCMC, assuming a specific distribution on the number of ICU beds occupied\\
    
    
    HMC:\\
    Sto comp \cite{flaxman2020report} (bayesian hierarchical model, parameters are estimated via adaptive HMC)\\
    
    ABC:\\
    Sto comp: \cite{chinazzi2020effect} ( 1) literature: range of latent period, infectious period, and generation time parameters; 2) data-driven: sensitivity analysis to select them with ABC and MAP with uniform prior for R0)
    
    Sequential MC:\\
    Sto comp \cite{kucharski2020early} (epidemio param, epidemic parameters; Erlang distribution for disease delays and exponential distribution for delay from onset to reporting)\\
    Sto stat: \cite{yang2020rational} and \cite{li2020estimation} (R0: sequential bayesian method, in which the posterior probability distribution of the R0 is estimated sequentially using the posterior at the previous time point as the new prior;)
    
    Incremental Mixture Importance Sampling \cite{zhangenns20}(Incremental Mixture Importance Sampling (bayesian algorithm) to estimate the a posteriori distribution of daily transmission rate given the ratio between asymptomatic and symptomatic per age (Russell et al.) (no more precisions))\\
    
    Sto comp/AB \cite{gleam2020modeling} \\
    
    Sto stat \cite{linton2020incubation} (pdf of the incubation period chosen as lognormal, Weibull, gamma distributions; bayesian method with the widely applicable information criterion (WAIC) for model selection; comparison with point estimation outputs from MLE)
    
    \item multinomial\\
     Sto comp \cite{wu2020nowcasting} (multinomial sampling process from the age distribution of true cases for the age distribution of confirmed cases)
\end{itemize}


